GaussianAvatar-Editor: Photorealistic Animatable Gaussian Head Avatar Editor

We introduce GaussianAvatar-Editor, an innovative framework for text-driven editing of animatable Gaussian head avatars that can be fully controlled in expression, pose, and viewpoint. Unlike static 3D Gaussian editing, editing animatable 4D Gaussian avatars presents challenges related to motion occlusion and spatial-temporal inconsistency. To address these issues, we propose the Weighted Alpha Blending Equation (WABE). This function enhances the blending weight of visible Gaussians while suppressing the influence on non-visible Gaussians, effectively handling motion occlusion during editing. Furthermore, to improve editing quality and ensure 4D consistency, we incorporate conditional adversarial learning into the editing process. This strategy helps to refine the edited results and maintain consistency throughout the animation. By integrating these methods, our GaussianAvatar-Editor achieves photorealistic and consistent results in animatable 4D Gaussian editing. We conduct comprehensive experiments across various subjects to validate the effectiveness of our proposed techniques, which demonstrates the superiority of our approach over existing methods. More results and code are available at: [Project Link](https://xiangyueliu.github.io/GaussianAvatar-Editor/).

==> sec/5_conclusion.tex <==
% \section{Conclusion}

% In this paper, we have presented GaussianAvatar-Editor, a text-driven framework for realistic animatable Gaussian avatar editing. For the motion occlusion problem where editing gradients would be back-propagated from non-occlusion parts to erroneously update the occlusion parts, we proposed a Weighted alpha blending equation (WABE) to replace the original Gaussian rendering function so as to suppress those erroneous updates. Moreover, to enhance the 4D supervision consistency of the editing supervision, we proposed an adversarial learning framework. By incorporating all these designs together, our method can produce high-quality, realistic editing results for 4D animatable Gaussian avatars. We have conducted comprehensive experiments on various subjects to validate the proposed methods. Both qualitative and quantitative results demonstrated that our method is superior to existing methods. 

% {\bf Limitations.} GaussianAvatar-Editor utilizes FLAME model to do animation, which could not animate unmodeled parts like the tongue. We leave this for future exploration.
